Weak radiative corrections to dijet production at the LHC

We summarize the calculation of the weak corrections to dijet production at hadron colliders, comprising tree-level effects of O(\alpha_s\alpha,\alpha^2) and loop corrections of O(\alpha_s^2\alpha). Although suppressed by the small value of the coupling constant \alpha, the weak radiative corrections can become large in the high-energy domain due to the appearance of Sudakov-type and other high-energy logarithms. Generally the corrections to the transverse-momentum distributions are larger by approximately a factor of two compared to the corresponding reach in the invariant-mass distributions, because the invariant-mass distributions are not, unlike the k_T distributions, dominated by the Sudakov regime at high scales. The electroweak tree-level contributions are found to be of the same generic size as the loop corrections.

==> feyndiags/TreeEW.tex <==
\begin{feynartspicture}(200,100)(2,1)
  \FADiagram{}
  \FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
  \FALabel(4.84577,13.4377)[t]{$\Pu$}
  \FAProp(0.,5.)(10.,6.)(0.,){/Straight}{1}
  \FALabel(5.15423,4.43769)[t]{$\Pd$}
  \FAProp(20.,15.)(10.,14.)(0.,){/Straight}{-1}
  \FALabel(14.8458,15.5623)[b]{$\Pu$}
  \FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
  \FALabel(15.1542,6.56231)[b]{$\Pd$}
  \FAProp(10.,14.)(10.,6.)(0.,){/Sine}{0}
  \FALabel(8.93,10.)[r]{$\gamma,\PZ$}
  \FAVert(10.,14.){0}
  \FAVert(10.,6.){0}

  \FADiagram{}
  \FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
  \FALabel(4.84577,13.4377)[t]{$\Pu$}
  \FAProp(0.,5.)(10.,6.)(0.,){/Straight}{1}
  \FALabel(5.15423,4.43769)[t]{$\Pd$}
  \FAProp(20.,15.)(10.,6.)(0.,){/Straight}{-1}
  \FALabel(16.8128,13.2058)[br]{$\Pu$}
  \FAProp(20.,5.)(10.,14.)(0.,){/Straight}{-1}
  \FALabel(17.6872,8.20582)[bl]{$\Pd$}
  \FAProp(10.,14.)(10.,6.)(0.,){/Sine}{-1}
  \FALabel(9.03,10.)[r]{$\PW$}
  \FAVert(10.,14.){0}
  \FAVert(10.,6.){0}
\end{feynartspicture}

